ViCLEVR: A Visual Reasoning Dataset and Hybrid Multimodal Fusion Model for Visual Question Answering in Vietnamese

In recent years, Visual Question Answering (VQA) has gained significant attention for its diverse applications, including intelligent car assistance, aiding visually impaired individuals, and document image information retrieval using natural language queries. VQA requires effective integration of information from questions and images to generate accurate answers. Neural models for VQA have made remarkable progress on large-scale datasets, with a primary focus on resource-rich languages like English. To address this, we introduce the ViCLEVR dataset, a pioneering collection for evaluating various visual reasoning capabilities in Vietnamese while mitigating biases. The dataset comprises over 26,000 images and 30,000 question-answer pairs (QAs), each question annotated to specify the type of reasoning involved. Leveraging this dataset, we conduct a comprehensive analysis of contemporary visual reasoning systems, offering valuable insights into their strengths and limitations. Furthermore, we present PhoVIT, a comprehensive multimodal fusion that identifies objects in images based on questions. The architecture effectively employs transformers to enable simultaneous reasoning over textual and visual data, merging both modalities at an early model stage. The experimental findings demonstrate that our proposed model achieves state-of-the-art performance across four evaluation metrics. The accompanying code and dataset have been made publicly accessible at \url{https://github.com/kvt0012/ViCLEVR}. This provision seeks to stimulate advancements within the research community, fostering the development of more multimodal fusion algorithms, specifically tailored to address the nuances of low-resource languages, exemplified by Vietnamese.

==> tex/Highlight.tex <==
\begin{highlights}
\item We introduce a novel visual reasoning dataset in Vietnamese (ViCLEVR).
\item We propose a hybrid visual reasoning methodology, integrating neural networks, transformers, and deep multimodal fusion with co-attention mechanisms (PhoViT)
\item Comprehensive analysis of the performance of five existing methods, including the proposed method, across various aspects. 
Our experiments and results show that ViCLEVR is the challenging dataset.
\end{highlights}

==> tex/ProblemForm.tex <==
\section{Problem statement}
\label{sec:prob}
The objective of Visual Question Answering (VQA) is to ascertain the most probable answer, given an image $I$ and a question $Q$, through the maximization of conditional probability using a computational model. To be more precise, when presented with an image $I$ and a question $Q$, the aim is to identify the answer $A$ that carries the highest probability from a set of potential answer choices $O$. This task can be formulated as the quest to discover the answer $A$ that maximizes the conditional probability $P(A|I,Q,O)$, expressed as follows:
\begin{equation}
A = \operatorname*{argmax}_{A\in O} P(A|I,Q,O)
\end{equation}
Indeed, the $\operatorname*{argmax}$ function returns the argument that maximizes the provided function.
The probability $P(A|I,Q,O)$ can be computed by utilizing a computational model that takes both the image $I$ and the question $Q$ as inputs and generates a probability distribution over the potential answer options in the set $O$. This distribution reflects the likelihood of each answer option given the provided image and question. The answer $A$ with the highest probability within this distribution is considered the most probable answer to the given question and image.
